Hierarchical Point Attention for Indoor 3D Object Detection

3D object detection is an essential vision technique for various robotic systems, such as augmented reality and domestic robots. Transformers as versatile network architectures have recently seen great success in 3D point cloud object detection. However, the lack of hierarchy in a plain transformer restrains its ability to learn features at different scales. Such limitation makes transformer detectors perform worse on smaller objects and affects their reliability in indoor environments where small objects are the majority. This work proposes two novel attention operations as generic hierarchical designs for point-based transformer detectors. First, we propose Aggregated Multi-Scale Attention (MS-A) that builds multi-scale tokens from a single-scale input feature to enable more fine-grained feature learning. Second, we propose Size-Adaptive Local Attention (Local-A) with adaptive attention regions for localized feature aggregation within bounding box proposals. Both attention operations are model-agnostic network modules that can be plugged into existing point cloud transformers for end-to-end training. We evaluate our method on two widely used indoor detection benchmarks. By plugging our proposed modules into the state-of-the-art transformer-based 3D detectors, we improve the previous best results on both benchmarks, with more significant improvements on smaller objects.

==> tables/3detr-sunrgbd.tex <==
\begin{table}[ht]
\begin{center}
\scalebox{0.7}{
\begin{tabular}{c|ll}
\toprule
Methods    & mAP@0.25 & mAP@0.50  \\
\hline
3DETR-m ($\texttt{epoch}$ 90$^{\ast}$) &   ~~~-~~~ (51.0)  &  ~~~-~~~ (22.0)  \\
3DETR-m ($\texttt{epoch}$ [90/1080]) &   43.9 (41.0)  &  13.2 (11.5)  \\
\hline
3DETR-m ($\texttt{epoch}$ [90/90]) &   51.7 (51.3)  &  22.6 (22.0)  \\
\rowcolor{LightCyan} w/ MS + Local (Ours)  &   52.3 (51.8) \textcolor{DarkGreen}{\small ($\uparrow 0.6$)}  &  23.6 (22.6) \textcolor{DarkGreen}{\small ($\uparrow 1.0$)} \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{\textbf{Reproducing 3DETR on SUN RGB-D.} ``$\ast$" denotes the official numbers provided by its authors. ``-" means the official result is not available. $\texttt{epoch}$ [a/b] is the model checkpoint at $a$ epoch while $b$ is the total number of training epochs.}
\label{tab:3detr-sunrgbd}
\end{table}

==> tables/ablate_modules.tex <==
\begin{table}[!ht]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{c|c|cc}
\toprule
 MS-A & Local-A & mAP@0.25 & mAP@0.50 \\
 \midrule
     -    &    -   &   68.6   &   51.8  \\
 \ding{52} &  -     &   68.9  &   \textbf{52.5}   \\
 -   &  \ding{52}  &   68.8   &    52.3  \\
 \ding{52}  &  \ding{52}  &  \textbf{69.0}   &   52.3 \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{\textbf{The stand-alone effect of our attention modules.} }
\vspace{-1em}
\footnotesize {The configuration in the first row denotes the Group-Free$^{12, 512}$ baseline. The results are averaged over 25 trials.}
\label{tab:ablate-attn}
\end{table}

==> tables/ablate_ms.tex <==
\begin{table}[!ht]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{l|cc}
\toprule
 Layers  & mAP@0.25 & mAP@0.25 \\
 \midrule
 $[0]$  &  \textbf{68.9}  &  \underline{52.5}  \\
 $[0, 4, 8]$  &  \underline{68.8}  &  52.4  \\
 $[0, 3, 6, 9]$  &  \textbf{68.9}  & 52.3  \\
 $[0, 2, 4, 6, 8, 10]$  & 68.7  & \textbf{52.6}  \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{\textbf{Different placements of the simple multi-scale attention layer.} Layers = $[i]$ means we replace the $i$\-th layer of the transformer decoder with our MS-A layer. The best results are in bold, and the second-best results are underlined. }
\label{tab:ablate-ms}
\end{table}

==> tables/analysis-size.tex <==
\begin{table}[!ht]
\caption{\textbf{Performance on different size categories on ScanNetV2.}}
\vspace{-1em}
\footnotesize {We define the S/M/L thresholds based on the statistics (volume distribution) of ScanNetV2 objects. The configuration in the first row denotes the Group-Free$^{12, 512}$ baseline. Results are averaged over 25 trials.}% \ning{Do we still have time to report the per-size mAP for each baseline, to show how poorly they perform on small objects?}}
\begin{center}
\scalebox{0.9}{
\begin{tabular}{c|c|lll}
\toprule
MS-A & Local-A & mAP$_S$ & mAP$_M$ & mAP$_L$ \\
 \midrule
    -     &   -      &   63.1  & 76.6  &  83.2  \\
 \ding{52}  & - &   65.0   & 77.5  &  83.9 \\
    -     &  \ding{52} & 65.1 & 77.9  & 83.4 \\
\ding{52}  &   \ding{52}   & \textbf{65.3} \textcolor{DarkGreen}{\small ($\uparrow 2.2$)} & \textbf{78.3} \textcolor{DarkGreen}{\small ($\uparrow 1.7$)} & \textbf{84.0} \textcolor{DarkGreen}{\small ($\uparrow 0.8$)} \\
 \bottomrule
\end{tabular}
}
\end{center}

\label{tab:analysis-size}
\end{table}

==> tables/class_scannet_ap25.tex <==
\begin{table*}[ht]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{l|c|cccccccccccccccccc|c}
\toprule
methods & backbone & cab & bed & chair & sofa & tabl & door & wind & bkshf & pic & cntr & desk & curt & fridg & showr & toil & sink & bath & ofurn & mAP \\ 
\hline
VoteNet~\cite{votenet} & PointNet++ & 47.7& 88.7 & 89.5 & 89.3 & 62.1 & 54.1 & 40.8 & 54.3 & 12.0 & 63.9 & 69.4 & 52.0 & 52.5 & 73.3 & 95.9 & 52.0 & 92.5 & 42.4 & 62.9 \\
H3DNet~\cite{h3dnet}& 4$\times$PointNet++ & 49.4 &88.6 &91.8 & 90.2 &64.9 & 61.0 &51.9& 54.9 & 18.6 &62.0 &75.9 &57.3 &57.2 &75.3 &97.9 &67.4 &92.5 &53.6 &67.2 \\ 
% 3DETR~\cite{3detr}& transformer & 50.2 & 87.0 &86.0 & 87.1 &61.6 &46.6 & 40.1 &54.5 & 9.1 &62.8 &69.5 &48.4 &50.9 &68.4 &97.9 &67.6 &85.9 &45.8 &62.7 \\ 
3DETR~\cite{3detr} & transformer & 49.4 & 83.6 &90.9 & 89.8 &67.6 &52.4 & 39.6 &56.4 & 15.2 &55.9 &79.2 &58.3 &57.6 &67.6 &97.2 &70.6 &92.2 &53.0 &65.0 \\ 
Pointformer~\cite{pointformer}& Pointformer & 46.7 &88.4 &90.5 & 88.7 & 65.7 & 55.0 &47.7& 55.8 & 18.0 &63.8 &69.1 &55.4 &48.5 &66.2 &98.9 &61.5 &86.7 &47.4 &64.1 \\
\hline
GroupFree$^{6, 256}$ & PointNet++ & 54.1 & 86.2& 92.0 & 84.8 & 67.8 & 55.8 & 46.9 & 48.5 & 15.0 & 59.4 & 80.4 & 64.2 & 57.2 & 76.3 & 97.6 &  76.8 & 92.5 & 55.0 & 67.3 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 55.9 & 88.6& 93.6 & 90.8 & 68.2 & 59.0 & 44.2 & 50.3 & 14.6 & 63.0 & 85.0 & 62.8 & 58.5 & 68.6 & 97.6 &  73.2 & 92.4 & 56.4 & 67.9 \\
RepSurf-U$^{6, 256}$ & PointNet++ & 55.5 & 87.7 & 93.4 & 85.9 & 69.1 & 57.3 & 48.8 & 50.0 & 16.5 & 61.0 & 81.6 & 66.2 & 59.0 & 77.5 & 99.2 & 78.2 & 94.0 & 56.8 & 68.8 \\ 
RepSurf-U$^{6, 256}$ (repd.) & PointNet++ & 57.4 & 89.6 & 93.2 & 87.4 & 70.2 & 58.8 & 46.6 & 47.4 & 18.1 & 63.4 & 78.2 & 70.4 & 46.5 & 81.0 & 99.8 & 69.4 & 90.8 & 55.5 & 68.0 \\ 
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 51.2 & 89.5 & 93.4 & 87.5 & 71.8 & 60.5 & 49.0 & 57.7 & 21.9 & 65.2 & 82.1 & 70.3 & 53.3 & 80.2 & 98.2 & 68.8 & 91.9 & 58.2 & 69.5 \\ 
\hline
GroupFree$^{12, 512}$ & PointNet++w2x & 52.1 &  91.9 &  93.6 & 88.0 & 70.7 & 60.7 &  53.7 &  62.4 & 16.1
& 58.5 & 80.9 &  67.9 & 47.0 &  76.3 &  99.6 & 72.0 &  95.3 &56.4  &  69.1 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 53.7 & 91.9& 93.4 & 88.8 & 72.1 & 61.3 & 52.8 & 58.6 & 17.4 & 70.8 & 83.3 & 69.9 & 56.5 & 75.6 & 98.5 &  70.3 & 94.4 & 56.9 & 70.3 \\
RepSurf-U$^{12, 512}$ & PointNet++w2x & 54.6 & 94.0 & 96.2 & 90.5 & 73.2 & 62.7 & 55.7 & 64.5 & 18.6 & 60.9 & 83.1 & 69.9 & 49.4 & 78.4 &  99.4 & 74.5 & 97.6 & 58.3 &  71.2 \\
RepSurf-U$^{12, 512}$ (repd.) & PointNet++w2x & 54.5 & 90.7 & 93.4 & 87.6 & 76.3 & 64.4 & 54.4 & 61.4 & 19.0 & 62.2 & 84.0 & 69.2 & 48.8 & 79.2 &  99.8 & 75.9 & 92.2 & 62.0 &  70.8 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++w2x & 58.0 &  89.3 &  94.1 & 86.5 & 74.3 & 62.4 &  60.2 &  57.9 & 21.7 & 67.9 & 85.3 &  74.4 & 53.5 &  75.9 &  99.6 & 74.6 &  91.6 &63.7  &  71.7 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Performance of mAP@0.25 in each category on ScanNetV2.}}
\label{tab:appendix-scannet-ap25}
\end{table*}

==> tables/class_scannet_ap50.tex <==
\begin{table*}[ht]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{l|c|cccccccccccccccccc|c}
\toprule
methods & backbone & cab & bed & chair & sofa & tabl & door & wind & bkshf & pic & cntr & desk & curt & fridg & showr & toil & sink & bath & ofurn & mAP \\ 
\hline
VoteNet~\cite{votenet} & PointNet++ & 14.6 & 77.8 & 73.1 &  80.5 & 46.5 & 25.1 & 16.0 & 41.8 & 2.5 & 22.3 & 33.3 & 25.0 & 31.0 & 17.6 & 87.8 & 23.0 & 81.6 & 18.7 & 39.9 \\
H3DNet~\cite{h3dnet}& 4$\times$PointNet++ & 20.5 &79.7& 80.1& 79.6& 56.2& 29.0& 21.3& 45.5 & 4.2& 33.5& 50.6& 37.3& 41.4& 37.0& 89.1& 35.1&  90.2& 35.4 & 48.1 \\
\hline
GroupFree$^{6, 256}$ & PointNet++ & 23.0 &78.4 &78.9 &68.7 &55.1 & 35.3 & 23.6 & 39.4 & 7.5 & 27.2 & 66.4 & 43.3& 43.0 & 41.2 & 89.7 & 38.0 & 83.4 & 37.3 & 48.9 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 27.3 &80.8 &83.3 &85.3 &60.2 & 39.7 & 21.7 & 40.4 & 7.6 & 41.7 & 61.5 & 42.9& 42.3 & 26.2 & 96.1 & 38.5 & 89.5 & 39.7 & 51.4 \\
RepSurf-U$^{6, 256}$ & PointNet++ & 24.9 & 79.6 & 80.1 & 70.4 & 56.4 & 36.7 & 25.5 & 41.4 & 8.8 & 28.7 & 68.0 & 45.2 & 45.0 & 42.7 & 91.3 & 40.1 & 85.1 & 39.2 & 50.5 \\
RepSurf-U$^{6, 256}$ (repd.) & PointNet++ 1. & 24.3 & 82.6 & 82.6 & 71.3 & 55.9 & 38.3 & 18.6 & 40.3 & 11.2 & 44.0 & 60.7 & 45.1 & 35.7 & 36.6 & 97.1 & 34.6 & 84.6 & 39.8 & 50.2 \\ 
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 27.1 & 80.9 & 83.0 & 77.1 & 58.0 & 45.8 & 24.8 & 50.8 & 10.5 & 31.9 & 67.7 & 44.6 & 40.6 & 34.9 & 97.7 & 38.3 & 87.3 & 44.6 & 52.5 \\ 
\hline
GroupFree$^{12, 512}$ & PointNet++w2x & 26.0 &  81.3 & 82.9 & 70.7 & 62.2 &  41.7 &  26.5 &  55.8 & 7.8 & 34.7 &  67.2 &  43.9&  44.3 &44.1 & 92.8 & 37.4 & 89.7 & 40.6 &  52.8 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 31.0 & 81.0& 85.0 & 79.4 & 61.1 & 44.5 & 27.9 & 50.6 & 10.1 & 45.0 & 61.2 & 54.1 & 39.5 & 43.5 & 91.7 &  45.9 & 89.3 & 42.4 & 54.6 \\
RepSurf-U$^{12, 512}$ & PointNet++w2x & 28.5 & 83.5 & 84.8 & 72.6 & 64.0 & 43.6 & 28.3 & 57.8 & 9.6 & 37.0 & 69.7 & 45.9 & 46.4 & 46.1 & 94.9 & 39.1 & 92.1 & 42.6 &  54.8 \\
RepSurf-U$^{12, 512}$ (repd.) & PointNet++w2x & 27.6 & 82.7& 85.3 & 68.8 & 60.6 & 44.0 & 27.3 & 56.7 & 9.6 & 39.6 & 63.7 & 53.8 & 43.0 & 42.4 & 99.8 &  38.8 & 88.7 & 47.3 & 54.4 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++w2x & 29.3 &  83.6 &  85.7 & 78.7 & 66.2 & 45.6 &  30.4 &  59.8 & 10.4 & 34.2 & 60.0 &  60.8 & 48.1 &  45.3 &  99.9 & 44.5 &  87.1 &48.4  &  56.5 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Performance of mAP@0.50 in each category on ScanNetV2.}}
\label{tab:appendix-scannet-ap50}
\end{table*}

==> tables/class_sunrgbd_ap25.tex <==
\begin{table*}[ht]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{l|c|cccccccccc|c}
\toprule
methods & backbone & bathtub & bed & bkshf & chair & desk & drser & nigtstd & sofa & table & toilet & mAP \\
\hline
VoteNet~\cite{votenet} & PointNet++ & 75.5 & 85.6 & 31.9 & 77.4 & 24.8 & 27.9 & 58.6 & 67.4 & 51.1 & 90.5 & 59.1\\
H3DNet~\cite{h3dnet}& 4$\times$PointNet++ & 73.8 &85.6 &31.0& 76.7 &29.6& 33.4& 65.5& 66.5& 50.8& 88.2& 60.1 \\
3DETR~\cite{3detr} & transformer & 69.8 &84.6 &28.5& 72.4 &34.3& 29.6& 61.4& 65.3& 52.6& 91.0& 61.1 \\
Pointformer~\cite{pointformer}& Pointformer & 80.1 &84.3 &32.0& 76.2 &27.0& 37.4& 64.0& 64.9& 51.5& 92.2& 61.1 \\
\hline
GroupFree$^{6, 256}$ & PointNet++ &  80.0 &  87.8 & 32.5  &  79.4 &32.6 &  36.0 &  66.7  &  70.0  &  53.8  & 91.1  &  63.0\\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ & 83.2 &  86.7 & 34.5  &  79.0 &31.9 &  39.3 &  66.0  &  70.6  &  55.6  & 90.8  &  63.8\\
RepSurf-U$^{6, 256}$ & PointNet++ &  81.1 & 89.3 & 34.4 & 80.4 & 33.5 & 37.3 & 68.1 & 71.4 & 54.8 & 92.3  &  64.3 \\
RepSurf-U$^{6, 256}$ (repd.) & PointNet++ &  79.5 & 87.5 & 33.8 & 79.4 & 32.7 & 40.2 & 69.0 & 70.3 & 55.4 & 92.1  &  64.0 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ &  79.9 & 87.0 & 36.8 & 79.5 & 33.8 & 41.4 & 67.4 & 71.2 & 55.3 & 92.4  &  64.5 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Performance of mAP@0.25 in each category on SUN RGB-D.}}
\label{tab:appendix-sunrgbd-ap25}
\end{table*}

==> tables/class_sunrgbd_ap50.tex <==
\begin{table*}[ht]
\begin{center}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\begin{tabular}{l|c|cccccccccc|c}
\toprule
methods & backbone & bathtub & bed & bkshf & chair & desk & drser & nigtstd & sofa & table & toilet & mAP \\
\hline
VoteNet~\cite{votenet} & PointNet++ & 45.4 & 53.4 & 6.8 & 56.5 & 5.9 & 12.0 & 38.6 & 49.1 & 21.3 & 68.5 & 35.8 \\
H3DNet~\cite{h3dnet}& 4$\times$PointNet++ & 47.6 &52.9 &8.6& 60.1 & 8.4& 20.6& 45.6& 50.4& 27.1& 69.1& 39.0 \\
\hline
GroupFree$^{6, 256}$ & PointNet++ &  64.0 &  67.1 &  12.4 &  62.6 & 14.5 &  21.9&  49.8&  58.2 &  29.2 &  72.2 &  45.2\\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ &  66.2 &  67.4 &  10.8 &  63.6 & 15.0 &  24.7&  56.7&  56.1 &  30.8 &  74.3 &  46.6\\
RepSurf-U$^{6, 256}$ & PointNet++ &  65.2 & 67.5 & 13.2 & 63.4 & 15.0 & 22.4 & 50.9 & 58.8 & 30.0 & 72.7 &  45.9\\
RepSurf-U$^{6, 256}$ (repd.) & PointNet++ &  61.4 & 66.8 & 11.3 & 64.0 & 14.8 & 24.2 & 51.8 & 59.0 & 31.6 & 71.7 & 45.7 \\
\rowcolor{LightCyan} w/ MS + Local & PointNet++ &  62.2 & 67.6 & 16.6 & 65.0 & 15.0 & 24.2 & 57.0 & 59.0 & 30.9 & 77.7 & 47.5 \\
\bottomrule
\end{tabular}
\end{center}
\caption{\textbf{Performance of mAP@0.50 in each category on SUN RGB-D.}}
\label{tab:appendix-sunrgbd-ap50}
\end{table*}

==> tables/inference-speed.tex <==
\begin{table}[h!]
\begin{center}
\scalebox{0.9}{
\begin{tabular}{c|c|cc}
\toprule
\multirow{2}{*}{MS-A} & \multirow{2}{*}{Local-A} & \#Params & Inference Speed  \\
& & (M) & (ms/frame)  \\
 \midrule
    -     &   -  &  29.56  &  262   \\
        -     &  \ding{52} &  29.56 (+0.0) & 266   \\
 \ding{52}  & - &  29.64 (+0.08)  &  333    \\
\ding{52}  &   \ding{52}   & 29.64 (+0.08) &  340   \\
 \bottomrule
\end{tabular}
}
\end{center}
\caption{\textbf{Ablating the parameter and computation overhead of individual attention modules.}}
\label{tab:inference-speed}
\end{table}

==> tables/main_table_merged.tex <==
\begin{table*}[ht]
\caption{\textbf{Performance of object detection on ScanNetV2 and SUN RGB-D.} }
\vspace{-1em}
\footnotesize {We follow the standard protocol~\cite{votenet} by reporting the best results over 5 $\times$ 5 trials (5 trainings, each with 5 testings) and including the averaged results in the bracket. Group-Free$^{L, O}$ denotes the variant with $L$ decoder layers and $O$ object candidates. The same notation applies to RepSurf-U. The detection code of RepSurf is not published, so we implement our version of RepSurf-U and apply our method to it. We include the results of our implementation of RepSurf-U. }
\begin{center}
\scalebox{0.8}{
\begin{tabular}{c|c|c|ll|ll}
\toprule
\multirow{2}{*}{Methods}    & \multirow{2}{*}{\#Params} & \multirow{2}{*}{Backbone}  & \multicolumn{2}{c}{ScanNet V2} & \multicolumn{2}{c}{SUN RGB\_D}  \\
\cmidrule(lr){4-5} \cmidrule(lr){6-7}
                            & &   & mAP@0.25 & mAP@0.50 & mAP@0.25 & mAP@0.50  \\
\midrule
VoteNet~\cite{votenet}    &   -    &  PointNet++ &  62.9  &  39.9  &  59.1  &  35.8  \\
H3DNet~\cite{h3dnet}     &   -    &  PointNet++ &  64.4   & 43.4 &  60.1  &  39.0 \\
H3DNet~\cite{h3dnet}     &   -    &  4$\times$PointNet++ & 67.2   & 48.1  & -   & -   \\
Pointformer~\cite{pointformer}  &   -    &  transformer &  64.1    &  42.6 &  61.1    &  36.6   \\
\hline 
3DETR-m~\cite{3detr} (reproduce)  &   7.44M    &  transformer &  64.1 (62.9)    &  45.8 (44.1) &  58.2    &  30.6   \\
\rowcolor{LightCyan} w/ MS + Local (Ours)      &   7.50M    &  transformer &    \textbf{64.8 (63.7)} \textcolor{DarkGreen}{\small ($\uparrow 0.7$)}  &    \textbf{46.4 (45.2)} \textcolor{DarkGreen}{\small ($\uparrow 0.6$)} &  & \\
\hline 
Group-Free$^{6, 256}$~\cite{groupfree} &  14.47M  &  PointNet++ &  67.3 (66.3)   &  48.9 (48.5)  &  63.0 (62.6)   &  45.2 (44.4)  \\
\rowcolor{LightCyan} w/ MS + Local (Ours)  &  14.55M  &  PointNet++  &    67.8 (66.8) \textcolor{DarkGreen}{\small ($\uparrow 0.5$)}  &    50.8 (49.5) \textcolor{DarkGreen}{\small ($\uparrow 1.9$)} &   63.3 (62.8) \textcolor{DarkGreen}{\small ($\uparrow 0.3$)}  &   45.8 (44.9) \textcolor{DarkGreen}{\small ($\uparrow 0.6$)}   \\
RepSurf-U$^{6, 256}$~\cite{ran2022surface}  &  14.51M   &  PointNet++ &  68.8 (  ~~-~  )  &  50.5 (  ~~-~  ) &  64.3 (  ~~-~  )  &  45.9 (  ~~-~  )   \\
RepSurf-U$^{6, 256}$ (reproduce)  &  14.51M   &  PointNet++ &  68.0 (67.4)   &  50.2 (48.7) &  64.0 (63.3)   &  45.7.2 (45.2)  \\
\rowcolor{LightCyan} w/ MS + Local (Ours)  &  14.59M  &  PointNet++   &    \textbf{69.9 (68.7)} \textcolor{DarkGreen}{\small ($\uparrow 1.9$)}   &    \textbf{53.0 (51.3)} \textcolor{DarkGreen}{\small ($\uparrow 2.8$)}  &   \textbf{64.2} (\textbf{63.6}) \textcolor{DarkGreen}{\small ($\uparrow 0.2$)}   &   \textbf{47.0} (\textbf{45.7}) \textcolor{DarkGreen}{\small ($\uparrow 1.3$)} \\
% \hline
% Group-Free$^{12, 512}$~\cite{groupfree} &  29.56M   &  PointNet++w2x &  69.1 (68.6)   & 52.8 (51.8) & & \\
% \rowcolor{LightCyan} w/ MS + Local (Ours)  &  29.64M &  PointNet++w2x &    70.3 (69.0) \textcolor{DarkGreen}{\small ($\uparrow 1.2$)}   &    53.5 (52.3) \textcolor{DarkGreen}{\small ($\uparrow 0.7$)}  & & \\
% RepSurf-U$^{12, 512}$~\cite{ran2022surface}  &  29.68M   &  PointNet++w2x & 71.2 (  ~~-~  )   & 54.8 (  ~~-~  )  & & \\
% RepSurf-U$^{12, 512}$ (reproduce)  &  29.68M   &  PointNet++w2x & 70.8 (70.2)   & 54.4 (53.6)  & & \\
% \rowcolor{LightCyan} w/ MS + Local (Ours)  &  29.76M &  PointNet++w2x &    \textbf{71.4 (70.6)} \textcolor{DarkGreen}{\small ($\uparrow 0.6$)}   &    \textbf{55.6 (54.3)} \textcolor{DarkGreen}{\small ($\uparrow 0.8$)}  & & \\

\bottomrule
\end{tabular}
}
\end{center}
% \footnotesize{}

\label{tab:main}
\end{table*}
